Hardness of Detecting Abelian and Additive Square Factors in Strings

We prove 3SUM-hardness (no strongly subquadratic-time algorithm, assuming the 3SUM conjecture) of several problems related to finding Abelian square and additive square factors in a string. In particular, we conclude conditional optimality of the state-of-the-art algorithms for finding such factors. Overall, we show 3SUM-hardness of (a) detecting an Abelian square factor of an odd half-length, (b) computing centers of all Abelian square factors, (c) detecting an additive square factor in a length-$n$ string of integers of magnitude $n^{\mathcal{O}(1)}$, and (d) a problem of computing a double 3-term arithmetic progression (i.e., finding indices $i \ne j$ such that $(x_i+x_j)/2=x_{(i+j)/2}$) in a sequence of integers $x_1,\dots,x_n$ of magnitude $n^{\mathcal{O}(1)}$. Problem (d) is essentially a convolution version of the AVERAGE problem that was proposed in a manuscript of Erickson. We obtain a conditional lower bound for it with the aid of techniques recently developed by Dudek et al. [STOC 2020]. Problem (d) immediately reduces to problem (c) and is a step in reductions to problems (a) and (b). In conditional lower bounds for problems (a) and (b) we apply an encoding of Amir et al. [ICALP 2014] and extend it using several string gadgets that include arbitrarily long Abelian-square-free strings. Our reductions also imply conditional lower bounds for detecting Abelian squares in strings over a constant-sized alphabet. We also show a subquadratic upper bound in this case, applying a result of Chan and Lewenstein [STOC 2015].

==> _fig_alg.tex <==
\begin{tikzpicture}
\draw[->] (0,0)--(0,1) node[midway,left] {$a$};
\draw[->,dotted] (4,3)--(4,4) node[midway,right] {$a+b$};
\draw[->] (0,0)--(4,3) node[midway,right] {$b$};
\draw[->] (0,0)--(2,2) node[midway,left] {$s$};
\draw[->,dotted] (2,2)--(4,4) node[midway,left] {$s'=2\cdot s$};


\foreach \c [count=\i] in {1,1,0,0,0,1,0,0,0,1} {
  \node (c\i) [above] at (\i*0.5,-1) {$\mathtt{\c}$};
}
\draw[->] (0.25,-1.1) -- (0.25+0.5*1,-1.1);
\node at (0.25,-1.1) [left] {$a=(0,1)$};

\draw[->] (0.25,-1.5) -- (0.25+0.5*4,-1.5);
\node at (0.25,-1.5) [left] {$s=(2,2)$};

\draw[->] (0.25,-1.9) -- (0.25+0.5*7,-1.9);
\node at (0.25,-1.9) [left] {$b=(4,3)$};

\draw[decorate,decoration={bumps,amplitude=0.2cm,segment length=2.95cm}] 
      (0.25+0.5,-0.5) -- +(6*0.5,0.0);

\end{tikzpicture}
